A-posteriori error estimates for systems of hyperbolic conservation laws

We provide rigorous and computable a-posteriori error estimates for first order finite-volume approximations of nonlinear systems of hyperbolic conservation laws in one spatial dimension. Our estimators rely on recent stability results by Bressan, Chiri and Shen and a novel method to compute negative order norms of residuals. Numerical experiments show that the error estimator converges with the rate predicted by a-priori error estimates.

==> 5_outlook.tex <==

\section{Outlook}
\label{sec:outlook}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

